VideoMV: Consistent Multi-View Generation Based on Large Video Generative Model

Generating multi-view images based on text or single-image prompts is a critical capability for the creation of 3D content. Two fundamental questions on this topic are what data we use for training and how to ensure multi-view consistency. This paper introduces a novel framework that makes fundamental contributions to both questions. Unlike leveraging images from 2D diffusion models for training, we propose a dense consistent multi-view generation model that is fine-tuned from off-the-shelf video generative models. Images from video generative models are more suitable for multi-view generation because the underlying network architecture that generates them employs a temporal module to enforce frame consistency. Moreover, the video data sets used to train these models are abundant and diverse, leading to a reduced train-finetuning domain gap. To enhance multi-view consistency, we introduce a 3D-Aware Denoising Sampling, which first employs a feed-forward reconstruction module to get an explicit global 3D model, and then adopts a sampling strategy that effectively involves images rendered from the global 3D model into the denoising sampling loop to improve the multi-view consistency of the final images. As a by-product, this module also provides a fast way to create 3D assets represented by 3D Gaussians within a few seconds. Our approach can generate 24 dense views and converges much faster in training than state-of-the-art approaches (4 GPU hours versus many thousand GPU hours) with comparable visual quality and consistency. By further fine-tuning, our approach outperforms existing state-of-the-art methods in both quantitative metrics and visual effects. Our project page is aigc3d.github.io/VideoMV.

==> sections/abstract.tex <==
\begin{abstract}
  We present AM-MV, a generative model modified from large video generative models for consistent multi-view generation based on images or text prompts. Videos are two-dimensional time-serial projections of a dynamic 3D world and perceive various physical phenomena. While rigid rotation serves as almost the simplest physical phenomenon in the real world, it is sufficient to reconstruct a rigid object from multi-view images. AM-MV makes a large video generative model able to generate a turnaround video by finetuning it on multi-view data and regularizing the multi-view output in a RAR(Reconstruct and Render) way. In contrast to several thousand GPU hours used to finetune an image-generative model for sparse views generation, AM-MV can generate 24 dense views and reach comparable performance in only 4 GPU hours. By further fine-tuning AM-MV and applying RAR-style regularization, AM-MV outperforms the existing state-of-the-art methods as a prior in various downstream tasks. We implement AM-MV based on open-source video generative models and we will release our code and pre-trained model for further research.
  % \keywords{First keyword \and Second keyword \and Third keyword}
\end{abstract}

==> sections/abstract_v2.tex <==
\begin{abstract}
\xiaodong{
Generating multi-view images based on text or single-image prompts is a critical capability for 3D content creation. In this paper, we propose a dense consistent multi-view generation model that is fine-tuned from off-the-shelf video generative models. Compared to 2D diffusion models, the video generative model is more suitable for multi-view generation because it naturally considers frame connections and enforces frame consistency through its temporal module. Moreover, the video generative models are trained on large-scale diverse video data which has covered dense multi-view generation situations in the pre-training stage, and therefore they have the potential to generate well. Furthermore, we introduce a \textit{3D-Aware Denoising Sampling} that employs a feed-forward reconstruction module to get an explicit global 3D model and then adopts a consistent sampling strategy that effectively involves images rendered from the global 3D model into the denoising sampling loop to improve the multi-view consistency of our model, which also provides a fast way to create 3D assets represented by 3D Gaussians within a few seconds.
}
In contrast to several thousand GPU hours used to finetune a 2D diffusion model for sparse views generation, Our method can generate 24 dense views and reach comparable performance in only 4 GPU training hours.
\weihao{training time or inference time? make it clear}
By further finetuning, our approach outperforms the existing state-of-the-art methods in both quantitative metrics and visual effects. We implement our method based on open-source video generative models, and we will release our code and pre-trained model for further research.


\end{abstract}

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
The creation of 3D content holds a crucial role in modern game design, virtual reality, and the movie industry. However, the current man-made manufacturing pipeline is time-consuming, and hard to keep up with the growing demand. Researchers have made substantial progress with directly fitting the 3D representation into the networks. The obvious insufficiency of these works is the limited amount of 3D data, which constrains the diversity of generation. Therefore, leveraging off-the-shell text-image alignment prior of 2D generative models becomes an inevitable measure. 

Among related works, pioneer works adopt Score Distillation Sampling(SDS) and carefully add direction-related keywords for 3D generation. Although 2D diffusion models can not provide accurate direction control by prompts and need a long time for optimization, these methods can obtain feasible results most of the time, except for artifacts and failures sometimes. The biggest challenge of single-view distillation is inconsistency between multi-view(The Janus problem).

To mitigate the Janus Problem, follow-up works(based on image or text prompt) choose to fine-tune the 2D generative models for multi-view generation first. Zero123 modifies a 2D generative model for Novel View Synthesis and can generate views under camera control. To further enhance the consistency, SyncDreamer adds depth-wise attention and generates 16 views in a single forward loop. However, the 16 views are fixed, limiting its applications to score distillation. MVDream can generate 4 orthogonal views simultaneously according to camera pose and leverage dense self-attention to correlate all views. However, the dense self-attention costs a massive memory, making it impossible to enlarge the number of views. The camera control can generalize to unseen views to some extent, but we find that it often lacks accurate camera control experimentally.


In contrast to single-image generative models, video generative models can produce sequential frames that represent projections of a dynamic 3D world. In the real world, the dynamics are produced according to physical principles. If we connect the dense multi-view as a turnaround video and assume the camera is static, the multi-view images become a rigid rotation which is extremely simple among other physical phenomena like elastic deformation, collision, or fluids. 

Therefore, with a pre-trained large video generative model, we only need to arouse its memory of rigid rotation using a 3D dataset for multi-view generation. We draw inspiration from it and propose to fine-tune a large video generative model for dense multi-view generation. By incorporating camera poses like the previous methods, we can achieve an infinite generation of views on the up-hemisphere with controllable camera poses, which is essential for SDS optimization. Moreover, the generated dense views are also sufficient for us to train a NeRF(NeuS) field or train a multi-view LRM. What surprises us in our implementation process is that we only need a small high-quality dataset(28K) and 4 GPU hours to achieve comparable performance with the state-of-the-art method MVDream(2300 GPU hours). This phenomenon again verifies our motivation to start from a video generative model and also points out a way to conduct 3D generation research under limited computation resources.

Secondly, we need to eliminate other physical dynamics learned by the video generative model, which requires us to enforce the 3D consistency among multi-view images. While we could adopt the depth-wise attention module like SyncDreamer without Out-Of-Memory(OOM), we find this attention mechanism indeed encourages multi-view consistency rather than enforcing it. To make our model 3D-aware and maintain the initial state of the video generative model, we add a latent neural reconstruction module to derive regularization on latent and enforce the multi-view consistency.

In summary, our contributions include: 1) We propose a novel dense multi-view image generation model that is fine-tuned from off-the-shell video generative models and outperforms SoTA methods with a training process of only 4 GPU hours. 2) We design a novel latent RAR module for consistent multi-view image generation, which further boosts the performance of our model. 3) We conduct extensive experiments on public benchmarks and draw several directions for future works in depth.


















% qiu version
% The creation of 3D content holds a crucial role in modern game design, virtual reality, and the movie industry. However, the scarcity of readily available 3D data and the time-consuming process of acquiring it through manual manufacturing pose significant obstacles in learning a strong 3D prior to produce high-quality 3D generations for current 3D generative models. 

% % prior work address what?
% Recently, advancements in the field of 3D generation have introduced inference-based models, such as Shape-E and LRM ~\cite{, Hong2023LRMLR}, which employ diffusion-based or transformer-based frameworks to directly predict a 3D representation trained on public 3D datasets. Yet, The generalization ability of 3D inference-based methods is limited due to the insufficient 3D training data. With respect to the field of 2D generation, the computer vision community has witnessed the powerful generation ability of the 2D diffusion model trained on large-scale datasets. Hence, some researchers attempt to directly generate a 3D model from the 2D diffusion model. Dreamfusion~\cite{poole2022dreamfusion} proposes Score Distillation Sampling (SDS) to distill pre-trained 2D diffusion models for creating 3D models without using any 3D data. While Dreamfusion demonstrates strong generalizable ability and enables us to create high-quality and rich 3D assets using the SDS technique, the generated results may suffer from multi-face problems due to the lack of multi-view consistency in the 2D diffusion model.
% \weihao{also time consuming}

% To make the 2D diffusion model have multi-view consistency ability, recent researchers fine-tuned the Stable Diffusion model on the 3D synthetic dataset. MVDream~\cite{Shi2023MVDreamMD} simultaneously generates self-rotated multi-view images of the same object, conditioned on the camera poses, which effectively alleviates the Janus problem in SDS optimization. Wonder3D~\cite{Long2023Wonder3DSI} first generates multi-view RGB-Noraml images conditioned on camera pose, and then promptly reconstruct the 3D model by the multi-view construction method learned from these generated images. These approaches imply that \emph{once we obtain a generation model with multi-view consistency, Janus problem in SDS-based methods will be alleviated, or we can quickly generate 3D assets through off-the-shelf multi-view reconstruction methods} 

% Nevertheless, fine-tuning a 2D diffusion model into a multi-view consistency diffusion model poses challenges because the 2D diffusion model naturally lacks spatial and temporary consistency. Moreover, to make the 2D diffusion model achieve multi-view consistency, we need to train an additional temporary or multi-view aware attention module within the 2D diffusion model from scratch, resulting in slow convergence.

% Taking the above concerns into account, instead of 2D diffusion models, we adopt large-scale video generative models as a pre-trained model. Compared to 2D diffusion models, video generative models are better suited for multi-view generation due to their inherent consideration of frame connections and enforcement of frame consistency through temporal modules. Moreover, video generative models are trained on a diverse range of video data, encompassing both dynamic and static scenes with varying camera motions. Those training datasets include various self-rotated object videos similar to multi-view training data, thereby unlocking their potential for multi-view generation.

% Similar to existing work, we fine-tune a pre-trained video generative model to dense multi-view generation, using a limited public high-quality 3D dataset. We incorporate camera poses, by adding camera embeddings as a residual to time embeddings for each view, enabling infinite view generation. 

% Unlike prior work that only depends on the multi-view attention module to enhance multi-view consistency, we propose a novel \emph{3D-Aware Denoise Sampling} to further improve multi-view consistency. Specifically, we employ a feed-forward-based model conditioned on multi-view images generated by VideoMV to explicitly generate 3D models. Subsequently, these generated 3D models are rendered to the corresponding view and replace the original images produced by VideoMV in the denoising loop.

% Our experiments demonstrate that a 3D-aware diffusion model, fine-tuned from a video generative model, exhibits higher efficiency compared to a 2D diffusion model. VideoMV achieves comparable performance to MVdream fine-tuned from the 2D diffusion model while only requiring 4 GPU hours, in contrast to the 2300 GPU hours needed by MVDream.



% In summary, our contributions include: 
% 1) We propose VideoMV which is fine-tuned from off-the-shelf video generative models, with strong multi-view consistency prior. 
% 2) we introduce a novel 3D-aware denoise sampling strategy to further improve the multi-view consistency of the generated image
% 3) Extensive experiments demonstrate that our method outperforms state-of-the-art approaches in both quantitative and qualitative results with respect to the generation of multi-view consistency.

==> sections/introduction_v2.tex <==
\section{Introduction}
\label{sec:intro}

% \xiaodong{The creation of 3D content plays a crucial role in modern game design, virtual reality, and the movie industry. However, the current manual manufacturing pipeline is time-consuming and requires professional skills from users. Therefore, technology that allows for easy acquisition of 3D assets by generating them from text descriptions or single images has garnered attention and developed rapidly.

% Inspired by diffusion models~\cite{ddpm, latentdiffusion} and large transformer models~\cite{dall-e} that have achieved success in 2D image generation, some works~\cite{point-e, shap-e} propose 3D diffusion models directly to learn a 3D distribution or adopt a transformer-based framework to learn a 3D representation using millions of 3D datasets. However, the generalization ability of these works is limited to the scale of the dataset. To address the insufficient 3D data issue, DreamFusion~\cite{poole2022dreamfusion} proposes Score Distillation Sampling (SDS) to distill pre-trained 2D diffusion models for creating 3D models without using any 3D data. Thanks to powerful diffusion models, they can generate high-quality and diverse 3D assets, but they may encounter multi-face multi-faces problem due to inconsistent multi-view generation. In this paper, we focus on improving multi-view consistency. Once we obtain a consistent multi-view generation model, we can use it to mitigate the multi-faces problem in SDS-based methods, or quickly generate 3D assets through multi-view reconstruction.

% Zero123~\cite{liu2023zero1to3} proposes generating multi-view images by fine-tuning a 2D diffusion model with additional camera pose as conditional information. Their impressive results show that large-scale 2D diffusion models, when fine-tuned with a limited dataset, can achieve strong zero-shot generalization capability. Many subsequent works follow this principle, keeping the architecture of the 2D diffusion model as unchanged as possible or slightly modifying it to facilitate the loading of powerful pre-trained weights, and designing additional modules to improve multi-view consistency. SyncDreamer~\cite{liu2023syncdreamer} constructs an extra 3D spatial feature volume and uses projected features to build a depth-wise attention layer to correlate multi-view features. However, it only generates 16 fixed viewpoint images, limiting its downstream applications such as 3D generation via SDS-based methods. MVDream~\cite{mvdream} reuses the pre-trained 2D self-attention weights for a 3D self-attention layer to establish multi-view connections. It can generate an arbitrary number of multi-view images simultaneously based on camera pose. However, dense 3D attention proposed in MVDream incurs high memory costs when generating multiple images and may lack accurate camera control.

% In this paper, we adopt large-scale video generative models instead of 2D diffusion models as strong 3D priors. Video generative models are often transformed from 2D diffusion models by inserting temporal layers and fine-tuned on large-scale video datasets to generate temporally coherent videos. Compared to 2D diffusion models, video generative models are more suitable for multi-view generation since they naturally consider frame connections and enforce frame consistency through their temporal modules. Moreover, video generative models are trained on diverse video data, including dynamic and static scenes with various camera motions, which cover dense multi-view generation situations in the pre-training stage. This gives them the potential to generate multi-view images. Inspired by supervised fine-tuning (SFT) in large language models (LLM), we can adapt a pre-trained video generative model to a specific downstream task, such as dense multi-view generation, using a limited high-quality 3D dataset. In this paper, we incorporate camera poses, similar to previous methods, by adding camera embeddings to the time embeddings for each view, enabling infinite view generation. Surprisingly, in our implementation process, we achieve comparable performance to the state-of-the-art method MVDream (2300 GPU hours) using only a small high-quality dataset (28K) and 4 GPU hours. This phenomenon validates our motivation to start from a video generative model and also highlights a way to conduct 3D generation research with limited computational resources.

% To further improve multi-view consistency, we adopt a global 3D representation produced by the reconstruction module to constrain all the generated views from the same object, and then render more consistent multi-view images to replace the original generated images in the denoising loop. Inspired by recent multi-view reconstruction works such as LGM, we adopt the feed-forward reconstruction manner to directly regress the parameters of 3D Gaussians including position, scale factor, rotation quaternion, opacity value, and color feature. The number of Gaussians is equal to the number of pixels in multi-view features. Using a collection of fused 3D Gaussians to represent a global 3D model, we can efficiently render high-resolution images and utilize its differentiable render properties to add additional image-level rendering loss in the denoising training step which further regularizes the video generative models to generate more consistent images. In our experiments, we initially attempted to exploit the latent spatial features produced by the denoising network of the video generative models as input to the reconstruction module to effectively predict the parameters of the 3D Gaussian, but we found that the rendered images are blurry. We guess the reason is that the latent space is highly compressed and it is difficult to learn the reconstruction module well in limited 3D data, therefore we use images decoded by video generative models as input to the reconstruction module. However, it may encounter efficiency issues due to passing through a decoder and encoder network. To address this issue, we propose a simple strategy of intermittently using rendered images to replace generated images in the denoising loop, to reduce the number of decoding and encoding. This is also reasonable since there is no need to use noisy results to reconstruct when in the early steps of the denoising loop. Furthermore, we can quickly get a global 3D model represented by 3D Gaussian Splatting within a few seconds. If we need to export a polygonal mesh, as similarly done in LGM, we can use generated dense views or rendered views from Gaussians to train an efficient NeRF which can be converted to a polygonal mesh, and it takes only about 1 minute.

% In summary, our contributions include: 1) We propose a novel dense multi-view image generation model that is fine-tuned from off-the-shell video generative models which provides strong 3D priors. 2) We introduce a global 3D representation through a feed-forward reconstruction module and adopt a consistent sampling strategy that effectively involves rendered images into the denoising sampling loop to further improve the multi-view consistency of our model, which also provides a fast way to create 3D assets represented by 3D Gaussians. 3) We conduct extensive experiments on public benchmarks and draw several directions for future works in depth.
% }



% Qiu method
% The creation of 3D content plays a crucial role in modern game design, virtual reality, and the movie industry. However, the current manual manufacturing pipeline is time-consuming and expensive, as the design of a comprehensive 3D asset necessitates the designer to possess proficient modeling skills. Therefore, technology facilitating effortless acquisition of 3D assets through textual descriptions or single images has garnered significant attention and undergone rapid development.







The creation of 3D content plays a crucial role in virtual reality, the game and movie industry, 3D design, and so on. However, the scarcity of large-scale 3D data and the high time consumption of acquiring it by hand pose significant obstacles in learning a strong 3D prior to produce high-quality 3D content for deep-learning-based generative models. 
Recent advancements like DreamFusion~\cite{poole2022dreamfusion} leverage the \textbf{2D generation prior} learned from large-scale image data to generate different views of the target object for the 3D generation. Despite of generating realistic views, such manners suffer from the Janus problem~\cite{} caused by the lack of 3D awareness in introducing 2D prior only. Subsequent works like MVDream~\cite{Shi2023MVDreamMD} and Wonder3D~\cite{Long2023Wonder3DSI} further learn from the limited 3D data~\cite{objaverse} to facilitate the multi-view consistency in the view generation process. But it is still ... [hard to keep or sacrifice the generation quality when forcing the multi-view consistency, slow to converge]

% prior work address what?
% Recently, advancements in the field of 3D generation have introduced inference-based models, such as Shape-E and LRM ~\cite{, Hong2023LRMLR}, which employ diffusion-based or transformer-based frameworks to directly predict a 3D representation trained on public 3D datasets. Yet, The generalization ability of 3D inference-based methods is limited due to the insufficient 3D training data. With respect to the field of 2D generation, the computer vision community has witnessed the powerful generation ability of the 2D diffusion model trained on large-scale datasets. Hence, some researchers attempt to directly generate a 3D model from the 2D diffusion model. Dreamfusion~\cite{poole2022dreamfusion} proposes Score Distillation Sampling (SDS) to distill pre-trained 2D diffusion models for creating 3D models without using any 3D data. While Dreamfusion demonstrates strong generalizable ability and enables us to create high-quality and rich 3D assets using the SDS technique, the generated results may suffer from multi-face problems due to the lack of multi-view consistency in the 2D diffusion model.
% \weihao{also time consuming}

% To make the 2D diffusion model have multi-view consistency ability, recent researchers fine-tuned the Stable Diffusion model on the 3D synthetic dataset. MVDream~\cite{Shi2023MVDreamMD} simultaneously generates self-rotated multi-view images of the same object, conditioned on the camera poses, which effectively alleviates the Janus problem in SDS optimization. Wonder3D~\cite{Long2023Wonder3DSI} first generates multi-view RGB-Noraml images conditioned on camera pose, and then promptly reconstruct the 3D model by the multi-view construction method learned from these generated images. These approaches imply that \emph{once we obtain a generation model with multi-view consistency, Janus problem in SDS-based methods will be alleviated, or we can quickly generate 3D assets through off-the-shelf multi-view reconstruction methods} 

Different from the existing attempts, we propose introducing the \textbf{video generation prior} learned from object-central videos to overcome the existing bottlenecks, for three reasons: (i) the data scale of object-central videos is large enough to learn a strong video generation prior; (ii) compared with 2D images, videos provide extra multi-view information of objects, so the video generation prior is promising to introduce 3D-aware knowledge into generation; (iii) views in a video present continuous and gradual changes that ease the cross-view association construction, which is important for the 3D shape learning.
In order to learn the video generation prior, we employ a video diffusion model that is learned from the video generation conditioned by a text or image guidance and a camera pose trajectory. 



Nevertheless, fine-tuning a 2D diffusion model into a multi-view consistency diffusion model poses challenges because the 2D diffusion model naturally lacks spatial and temporary consistency. Moreover, to make the 2D diffusion model achieve multi-view consistency, we need to train an additional temporary or multi-view aware attention module within the 2D diffusion model from scratch, resulting in slow convergence.

Taking the above concerns into account, instead of 2D image diffusion models, we adopt large-scale video generative models as the pre-trained model. Compared to 2D diffusion models, video generative models are better suited for multi-view generation due to their inherent consideration of frame connections and enforcement of frame consistency through temporal modules. Moreover, video generative models are trained on a diverse range of video data, encompassing both dynamic and static scenes with varying camera motions. Those training datasets include various self-rotated object videos similar to multi-view training data, thereby unlocking their potential for multi-view generation.

Similar to existing work, we fine-tune a pre-trained video generative model for dense multi-view generation, using a limited public high-quality 3D dataset. We incorporate camera poses by adding the camera embedding as a residual to the time embedding for each view, enabling infinite view generation. 

Unlike prior work that only depends on the multi-view attention module to enhance multi-view consistency, we propose a novel \emph{3D-Aware Denoise Sampling} to further improve the multi-view consistency. Specifically, we employ a feed-forward-based model conditioned on multi-view images generated by VideoMV to explicitly generate 3D models. Subsequently, these generated 3D models are rendered to the corresponding view and replace the original images produced by VideoMV in the denoising loop.

In the experiments, we demonstrate that a 3D-aware diffusion model, fine-tuned from a video generative model, exhibits higher efficiency compared to a 2D diffusion model. 
\weihao{compared to who? cite it. efficiency in which task? state it. Is the compared method really a 2D diffusion model?}
Our method achieves comparable performance with MVDream~\cite{} with only 4 GPU hours, while MVDream consumes 2300 GPU hours.
% , which is fine-tuned from the 2D diffusion model while only requiring 4 GPU hours, in contrast to the 2300 GPU hours needed by MVDream.



In summary, our contributions include: 
1) We propose VideoMV, which is fine-tuned from off-the-shelf video generative models, with strong multi-view consistency prior. 
2) we introduce a novel 3D-aware denoise sampling strategy to further improve the multi-view consistency of the generated image
3) Extensive experiments demonstrate that our method outperforms state-of-the-art approaches in both quantitative and qualitative results with respect to the generation of multi-view consistency.


\weihao{Claim: video generative models are more multi-view consistent. Prove this, or cite from other papers.}




==> sections/supp_mm_train.tex <==
\section{Multi-domain Generation}
Applying VideoMV to multi-domain generation is easy. We show the training process of our multi-domain multi-view generation using the cross-domain attention module in Wonder3D~\cite{Long2023Wonder3DSI}. As depicted in \cref{fig:supp_rgbnd}, multi-domain data are aligned coherently, which is especially beneficial for downstream 3D reconstruction pipelines as demonstrated in \cite{Long2023Wonder3DSI}. In the future, we will focus on how to recover better geometry and texture based on the dense multi-view images generated by VideoMV.

\begin{figure}[htbp]
% \vspace{-1.0em}
  \centering
  \includegraphics[width=1.0\linewidth]{supp_figs/supp_rgbnd.pdf}
  \caption{Visual results of the training process of multi-modal generation.}
  \label{fig:supp_rgbnd}
% \vspace{-2.0em}
\end{figure}

% \section{}
